Lifelong Neural Topic Learning in Contextualized Autoregressive Topic Models of Language via Informative Transfers

Topic models such as LDA, DocNADE, iDocNADEe have been popular in document analysis. However, the traditional topic models have several limitations including: (1) Bag-of-words (BoW) assumption, where they ignore word ordering, (2) Data sparsity, where the application of topic models is challenging due to limited word co-occurrences, leading to incoherent topics and (3) No Continuous Learning framework for topic learning in lifelong fashion, exploiting historical knowledge (or latent topics) and minimizing catastrophic forgetting. This thesis focuses on addressing the above challenges within neural topic modeling framework. We propose: (1) Contextualized topic model that combines a topic and a language model and introduces linguistic structures (such as word ordering, syntactic and semantic features, etc.) in topic modeling, (2) A novel lifelong learning mechanism into neural topic modeling framework to demonstrate continuous learning in sequential document collections and minimizing catastrophic forgetting. Additionally, we perform a selective data augmentation to alleviate the need for complete historical corpora during data hallucination or replay.

==> outline.tex <==
% !TEX root = ../main.tex
\clearemptydoublepage

\phantomsection
\addcontentsline{toc}{chapter}{Outline of the Thesis}

\begin{center}
	\huge{Outline of the Thesis}
\end{center}


%--------------------------------------------------------------------
\section*{Part I: Introduction and Theory}

\noindent {\scshape Chapter 1: Introduction}  \vspace{1mm}

\noindent  This chapter presents an overview of the thesis and it purpose. Furthermore, it will discuss the sense of life in a very general approach.  

\noindent {\scshape Chapter 2: Theory}  \vspace{1mm}

\noindent  No thesis without theory.   \vspace{1mm}

%--------------------------------------------------------------------
\section*{Part II: The Real Work}

\noindent {\scshape Chapter 3: Overview}  \vspace{1mm}

\noindent  This chapter presents the requirements for the process.
%--------------------------------------------------------------------
\section*{Part III: Future Work}

\noindent {\scshape Chapter 3: Overview}  \vspace{1mm}

\noindent  This chapter presents the requirements for the process.


==> preface.tex <==
% !TEX root = ../main.tex
\clearemptydoublepage
\phantomsection
\addcontentsline{toc}{chapter}{Preface}	


\vspace*{3cm}

\begin{flushleft}
{\Large \bf Preface}
\end{flushleft}

\vspace{1cm}




\newpage
